Jointly Measuring Diversity and Quality in Text Generation Models

Text generation is an important Natural Language Processing task with various applications. Although several metrics have already been introduced to evaluate the text generation methods, each of them has its own shortcomings. The most widely used metrics such as BLEU only consider the quality of generated sentences and neglect their diversity. For example, repeatedly generation of only one high quality sentence would result in a high BLEU score. On the other hand, the more recent metric introduced to evaluate the diversity of generated texts known as Self-BLEU ignores the quality of generated texts. In this paper, we propose metrics to evaluate both the quality and diversity simultaneously by approximating the distance of the learned generative model and the real data distribution. For this purpose, we first introduce a metric that approximates this distance using n-gram based measures. Then, a feature-based measure which is based on a recent highly deep model trained on a large text corpus called BERT is introduced. Finally, for oracle training mode in which the generator's density can also be calculated, we propose to use the distance measures between the corresponding explicit distributions. Eventually, the most popular and recent text generation models are evaluated using both the existing and the proposed metrics and the preferences of the proposed metrics are determined.

==> joinly measure arxive submit/figs/1.tex <==
\begin{figure*}[!thb]
    \centering
    \begin{subfigure}[b]{0.40\textwidth}
        \centering
        \includegraphics[width=0.93\textwidth]{plots/qualty_diversity/1_COCOCaptions.pdf}
    	\caption{\textit{COCO Captions} dataset}
    	\label{M2:coco}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.40\textwidth}
        \centering
    	\includegraphics[width=0.93\textwidth]{plots/qualty_diversity/1_EMNLP2017WMTNews.pdf}
    	\caption{\textit{EMNLP2017 WMT News} dataset}
    	\label{M2:emnlp}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.40\textwidth}
    	\centering
    	\includegraphics[width=0.93\textwidth]{plots/qualty_diversity/1_IMDBMovieReviews.pdf}
    	\caption{\textit{IMDB} dataset}
    	\label{M2:imdb}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.40\textwidth}
    	\centering
    	\includegraphics[width=0.93\textwidth]{plots/qualty_diversity/1_Oracle.pdf}
    	\caption{\textit{Oracle} dataset}
    	\label{M2:oracle}
    \end{subfigure}
    
    \caption{
    Diversity vs. quality measure of various models with temperatures from $1.5^{-3}$ to $1.5^4$ on different datasets. Each point in the plot corresponds to the performance of a model in a special temperature (A second-degree polynomial has been fitted to the points). Lower values in both axes show better ones.
    %Diversity measure (Self-BLEU4 for real data and  $-1\times$Entropy for synthetic data) against the quality measure ($1-$BLEU4 for real data and Oracle-NLL for synthetic data)} of various models with temperatures from $1.5^{-3}$ to $1.5^4$ on different datasets. Each point in the plot corresponds to the performance of a model in a special temperature (A second-degree polynomial has been fitted to the points). Lower values in both axes are better.
    }
    \label{M2:all}
\end{figure*}

==> joinly measure arxive submit/figs/2.tex <==
\begin{figure*}[!thb]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        % \includegraphics[trim={1.8cm 0 0.6cm 0}, clip,width=1\textwidth]{plots/real_metrics/2_NLL.pdf}
        \includegraphics[trim={0 0 0 0}, clip,width=1\textwidth]{plots/real_metrics/2_NLL_whithoutlegend.pdf}
    	\caption{NLL}
    	\label{M7:Nll}
    \end{subfigure}
    \,
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        % \includegraphics[trim={1.7cm 0 0.6cm 0}, clip, width=1\textwidth]{plots/real_metrics/2_1-MS-Jaccard4.pdf}
        \includegraphics[trim={0 0 0 0}, clip, width=1\textwidth]{plots/real_metrics/2_1-MS-Jaccard4_whithoutlegend.pdf}
    	\caption{MS-Jaccard4}
    	\label{M7:Jaccard}
    \end{subfigure}
    \,
    \begin{subfigure}[b]{0.36\textwidth}
    	\centering
        \includegraphics[trim={1.55cm 0 0.6cm 0}, clip, width=1\textwidth]{plots/real_metrics/2_FBD.pdf}
    	\caption{FBD}
    	\label{M7:FBD}
    \end{subfigure}

    \caption{NLL, $1-$MS-Jaccard4, and FBD scores of all the models without applying temperature (i.e. $T=1$) on different datasets. Lower values show better performance. %The order of the bars from left to right is the same as the order of the model names in legend from top to bottom; except to Fig. \ref{M7:Nll} (NLL) in which the NLL score for \textit{Real} is not present since we do not have a model for real data.
    \label{M7:allreal}
   }
\end{figure*}

==> joinly measure arxive submit/figs/3.tex <==
%%%%%%%%%%%%%% Oracle Distance %%%%%%%%%%%%%%%
\begin{figure}[!htb]
	\centering
	\includegraphics[trim={0.5cm 1cm 0.5cm 0}, clip,width=0.5\textwidth]{plots/3.pdf}
	\caption{The performance of all models (without applying temperature, i.e. $T=1$) on the Oracle dataset using different measures. Lower values show better performance.}
	\label{M7:Oracle_distance}
\end{figure}

==> joinly measure arxive submit/figs/4.tex <==
%%%%%%%%%%%%% Coor  %%%%%%%%%%%%%%%
\begin{figure}[!htb]
	\centering
% 	\includegraphics[trim={0.67cm 0 0 0},clip,width=0.57\textwidth]{plots/All_allk_M6_selected_pearson_Real.pdf}
	\includegraphics[trim={0 0 7.0cm 0},clip,width=0.5\textwidth]{plots/4.pdf}
	\caption{Pearson correlation of all metrics when aggregating results on the real world text datasets and all temperatures.}
	\label{M6:all}
\end{figure}
